Free-riders in Federated Learning: Attacks and Defenses

Federated learning is a recently proposed paradigm that enables multiple clients to collaboratively train a joint model. It allows clients to train models locally, and leverages the parameter server to generate a global model by aggregating the locally submitted gradient updates at each round. Although the incentive model for federated learning has not been fully developed, it is supposed that participants are able to get rewards or the privilege to use the final global model, as a compensation for taking efforts to train the model. Therefore, a client who does not have any local data has the incentive to construct local gradient updates in order to deceive for rewards. In this paper, we are the first to propose the notion of free rider attacks, to explore possible ways that an attacker may construct gradient updates, without any local training data. Furthermore, we explore possible defenses that could detect the proposed attacks, and propose a new high dimensional detection method called STD-DAGMM, which particularly works well for anomaly detection of model parameters. We extend the attacks and defenses to consider more free riders as well as differential privacy, which sheds light on and calls for future research in this field.

==> outline.tex <==
Attacks (weights generation):
    1. 0
    2. random
        a. with a variance similar to other clients' weights? (not really possible in real-world -- use fake data to train model and guess variance)
    3. diff of previous two rounds
        a. add noise such that the variance is similar to other clients' weights?
    
Defenses:
        a. add a global learning rate
            0.1/3/7/9
    1. variance
        a. other stats besides variance?

//    2. autoencoder?
//    3. DAGMM?
    4. can we detect fake generated weights without comparing with peer clients?
  To vary:
    1. detect at a single round: 0/10
        a. vary detection at begin - middle - end round
        b. should prefer early detection
    2. detect based on average weights of all rounds so far
    


To vary:
    1. With dp, repeat previous steps
        a. challenge - if a free-rider only appears 1 out of n rounds?


    4. ratios of free-riders
    
todo:
    dagmm + variance
    2. different training datasets and models
        a. especially, finding some combination that trains slow, so the begin-middle-end stage is clear.
    3. training data are evenly distributed to clients, or not

    detect free-riders from 100 variances:
        gaussian, clustering
        

vary: **detection period non-converge / converge
    a. evenly distributed
    b. **non-evely distributed - could be easier to detect based on variance

//1. toy example: A: 0 - D: sum weights 0??
2. A: random generated weights - D: autoencoder
//D: global validation dataset (ref: multi-KRUM on page2 //in https://arxiv.org/pdf/1811.09904.pdf)
3. A: diff of two previous rounds - D: global lr + variance [choices of lr - list values of variances]
4. A: diff of two previous rounds + fake data train model to guess variance - defense? DAGMM+variance?? (baseline: DAGMM, variance) randomly sample some clients for training each time
    a. verify of fake data model var is similar to others;
    b. if so, add variance of fake-model-var - two-prev-rounds-var
5. dp: 1A/2A/3A - 3D


I proposed a new outline:
1. A: random generated weights - D: DAGMM
//D: global validation dataset (ref: multi-KRUM on page2 //in https://arxiv.org/pdf/1811.09904.pdf)
3. A: diff of two previous rounds - D: global lr + variance-DAGMM [choices of lr - list values of variances]
4. A: diff of two previous rounds + fake data train model to guess variance - defense? DAGMM+variance?? (baseline: DAGMM, variance) randomly sample some clients for training each time
    a. verify of fake data model var is similar to others;
    b. if so, add variance of fake-model-var - two-prev-rounds-var
5. dp: 1A/2A/3A - 3D
